Capacitated Vehicle Routing with Target Geometric Constraints

We investigate the capacitated vehicle routing problem (CVRP) under a robotics context, where a vehicle with limited payload must complete delivery (or pickup) tasks to serve a set of geographically distributed customers with varying demands. In classical CVRP, a customer location is modeled as a point. In many robotics applications, however, it is more appropriate to model such "customer locations" as 2D regions. For example, in aerial delivery, a drone may drop a package anywhere in a customer's lot. This yields the problem of CVRG (Capacitated Vehicle Routing with Target Geometric Constraints). Computationally, CVRP is already strongly NP-hard; CVRG is therefore more challenging. Nevertheless, we develop fast algorithms for CVRG, capable of computing high quality solutions for hundreds of regions. Our algorithmic solution is guaranteed to be optimal when customer regions are convex. Numerical evaluations show that our proposed methods significantly outperform greedy best-first approaches. Comprehensive simulation studies confirm the effectiveness of our methods.

==> 03-cvrpbd.tex <==
\def\cvrpdp{\textsc{Alg-DP-CVRP}\xspace}
\def\cvrpdps{\textsc{DP-CVRP}\xspace}
\def\cvrpdpfh{\textsc{Alg-FH-DP-CVRP}\xspace}
\def\cvrpdpfhs{\textsc{FH-CVRP}\xspace}

In this section, we first describe an {\em exact} and {\em combinatorial} 
algorithm for tackling \cvrp, which runs in time $O(4^n)$. By 
further bounding the \emph{look-ahead horizon}, a high quality sub-optimal 
algorithm is obtained that runs in $O(n4^h)$, where $h$ is the look-ahead
horizon. We also briefly describe a non-combinatorial exact method based on 
branch-and-cut and a greedy algorithm that are used for comparison. 

\subsection{Exact and Finite-Horizon Combinatorial Algorithms}
\noindent\textbf{Exact combinatorial algorithm}.
Our exact algorithm for \cvrp proceeds in two phases. In the first phase, 
we exhaustively compute the optimal costs of all valid tours starting 
from the depot that visits a subset of customers. It is easy to see 
that there are at most $2^n$ tour combinations, many of which will be 
invalid as they will exceed the capacity limit. For each valid tour 
combination, the optimal cost is computed using an exact \tsp solver
\cite{simonetti1996implementation}. The costs are then stored for the 
second phase of the computation. 

In the second phase, to select the optimal set of disjoint tours, 
a straightforward application of dynamic programming (DP) is used. 
Let $C$ be the set of all customers. Let $I \subset C$ be the set of 
customers that have not been served and let $S_I$ be the set of customer subsets that can be visited in a single tour without violating the capacity constraint. Let $J_I$ be the optimal cost (i.e., the 
minimum total path length) to satisfy the demands of all of $I$, the 
standard DP recursion is 

\begin{align}
\label{eq:cvrpdp}
J_I = \min_{s \in S_I}(J_{I-s} + J_s). 
\end{align}

Note that $J_s$ is provided by the first phase through a direct look-up. 
The DP algorithm provides significant computational savings by storing 
the optimal cost of all possible $I$'s. For $n$ customers, there are 
at most $2^n$ such $I$'s. The algorithm, denoted \cvrpdp, is straightforward 
to implement: we simply create a large enough table to hold the $2^n$
entries and then iteratively populate the entries. 

\noindent\textbf{Algorithm analysis}. In the first phase, there are at 
most $2^n$ tours to examine. Since each tour visits no more than $n$ 
elements, obtaining the optimal cost of a tour takes $O(T(n))$ 
time, where $T(n)=O(2^n)$ even with a brute force TSP solver. 
The first phase then takes time $O(2^nT(n))$.

In the second phase, the incremental DP computation needs 
to go through $2^n$ possible $I$'s, starting from $I = \varnothing$ 
and eventually reach $I = C$. For each $I$, $S_I$ contains $O(|I|^k)$ 
potential tours that need to be checked. The second phase then 
requires $O(2^n 2^n)$, which dominates the computation time of the first 
phase. The overall computational complexity of \cvrpdp is then bounded 
by $O(2^{2n}) = O(4^n)$. 

With the application of DP cutting down the computation from a naive 
$O(n!f(n))$ (where $f(n)$ is some polynomial function of $n$ for 
computing the optimal cost of a single sequence) to $O(4^n)$, 
significantly larger \cvrp instances can be solved optimally. As we 
will demonstrate, \cvrpdp is exact. More importantly, \cvrpdp 
readily allows the integration of additional geometric constraints 
in the \cvrg formulation.

\textbf{Finite-horizon heuristic}. While \cvrpdp computes exact 
solutions with decent performance, the computation time is still 
exponential with respect to $n$. To address this issue, we introduce 
a finite horizon heuristic which restricts the number of customers 
examined at any given time. That is, some fixed $h$ ($h \le n$) customers 
are selected on which \cvrpdp is run. Because high quality solutions to 
\cvrp are generally clustered (see, e.g., Fig.~\ref{fig:setup} and 
Fig.~\ref{fig:cvrgExample}), these $h$ 
candidates are selected in a way to facilitate such clustering. 
%\jy{Need to add a reference to a \cvrp solution, and possibly add 
%additional explanation on how to select the $h$ candidates.}
%
From running \cvrpdp on the $h$ candidates, we pick two most "convenient" tours with 
the least average cost (path length/number of served customers), serve these customers, and repeat the process on 
the remaining customers. The heuristic algorithm, which we denote as 
\cvrpdpfh, has an apparent complexity of $O(n4^h)$, which is polynomial. 

\subsection{Other Methods}
For validating and comparing our algorithms, we examined the current literature 
on methods for solving \cvrp. Most existing algorithms appear to be based on 
branch-and-bound and branch-and-cut, e.g., \cite{laporte1986exact,
laporte1987exact,miller1995matching,toth1997exact,padberg1991branch,
caprara1997branch,blasum2000application,baldacci2004exact}. We selected one 
of the high-performance solvers, the VRP Solver \cite{pessoa2019generic}, 
based on branch-cut-and-price. We note that the VRP Solver cannot readily 
accommodate the geometric constraints in \cvrg. 

To evaluate the utility of our exact and near-optimal algorithms, a greedy 
algorithm is also implemented that simply starts a tour heading to the closest 
customer whose demand has not been met. The robot then keeps going to closest 
customers for delivery until the robot cannot visit more customers during that 
tour due to its capacity, at which point it returns to the depot. 


==> 05-cvrpbdgo.tex <==
\def\cvrgodp{\textsc{Alg-DP-CVRGO}\xspace}

In this section, we describe a heuristic algorithm for \cvrgo 
based on dynamic programming with guaranteed optimality upper 
bound. 

\subsection{Heuristic Algorithm based on Dynamic Programming}
In \cvrg, the distance between two polygonal objects are not affected
by other objects in between. This is no longer the case in \cvrgo, 
which makes the DP approach for \cvrg more challenging to apply. 
When we put the problem into the DP framework, the $c_s$ in~\eqref{eq:cvrpdp}
should be changed into $c_{s,I\backslash s}$ because when we compute 
the optimal path to pick up a one-tour set of objects, we need to 
consider the other objects remaining in the workspace as 
obstacles. 

\begin{align}
J_I = \min_{s\subseteq S_I} (J_{I\backslash s} + c_{s,I\backslash s})
\end{align}

The sub-problem of \cvrgo is then: given the one-tour set $s$ with 
obstacle set $(I\backslash s)$ in the workspace, find the optimal 
route to remove $s$.
%
The difficulty on the distance measurement and the dependence of the 
sub-problem on the original problem makes it computationally prohibitive 
to design an exact algorithm for \cvrgo. We address the issue by sampling
\emph{representative points} on the objects. These points are 
potential locations to be accessed by the robot. This transform the 
sub-problem into a graph-based \emph{generalized traveling salesperson 
problem} (GTSP) \cite{henrylab1969record}.

\begin{comment}
\begin{figure}[H]
    \centering
    \captionsetup{font={footnotesize}}
    \includegraphics[width=0.4\textwidth]{formatting/Figures/discretization.png}
    \caption{}
    \end{figure}
\end{comment}

Consider a graph $G=(V,E)$. For each edge $e \in G$, $c_e$ is the cost 
of using the edge. In GTSP, $V = S_1 \cup \ldots \cup S_{\ell}$ where 
$S_1, \ldots, S_{\ell}$ are pairwise disjoint. The goal is to find the 
lowest cost tour visiting each $S_i, 1 \le i \le \ell$ at least 
once. 
%
In our sub-problem, $m$ representative points are evenly sampled on each 
object. We can consider all the representative points on object $i$ as a set 
of vertices $S_i$ of GTSP. The depot is a single-element set. To solve the 
GTSP, we use the ILP model from \cite{laporte1987generalized}. We denote 
the high level DP procedure with GTSP based tour computation as \cvrgodp. 

\subsection{Upper Bound of \cvrgodp}
Given an instance $(I,s)$ of the sub-problem of \cvrgo and the number of 
samples $m$, we denote $R_{(I,s)}(m)$ to be the route computed by the GTSP
routine. $OPT_{(I,s)}$ is defined as the optimal cost. Using $\|\cdot \|$ 
to denote the cost of a route, we clearly have

%\jy{This is not very meaningful as a theorem - I am changing it to an 
%observation and commented out the proof.}
\begin{observation}
$\lim_{m \rightarrow \infty} \|(R_{(I,s)}(m))\| = OPT_{(I,s)}.$
\end{observation}
\begin{comment}
\begin{proof}
Denote $OPT_{(I,s)}(m)$ as the path that shares the same task sequence and the same way to avoid obstacles as $OPT_{(I,s)}$ but chooses pickup points among the same representative points as $R_{(I,s)}(d)$.\\

Since $R_{(I,s)}(d)$ is the solution of \cvrgodp when $d$ is fixed, we have $$\|R_{(I,s)}(d)\|\leq\|OPT_{(I,s)}(d)\|$$

According to the optimality of $OPT_{(I,s)}$, $$\|OPT_{(I,s)}\|\leq \|R_{(I,s)}(d)\|$$

Therefore, $$\|OPT_{(I,s)}\| \leq \|R_{(I,s)}(d)\| \leq\|OPT_{(I,s)}(d)\|$$

Since
$$ \lim_{d\rightarrow \infty} \|OPT_{(I,s)}(d)\|=\|OPT_{(I,s)}\|$$

we can obtain the conclusion of the theorem.
$$ \lim_{d \rightarrow \infty}\|R_{(I,s)}(d)\| = \|OPT_{(I,s)}\|$$
\end{proof}
\end{comment}

For a given discretization level, we can also bound the possible 
optimality loss. 

\begin{proposition}
Assuming the largest object perimeter is $L$, we have $\|R_{(I,s)}(m)\| 
\leq OPT_{(I,s)} + \dfrac{|s|L}{m}$.
\end{proposition}

\begin{proof}
Given object with perimeter length $L$, the distance between adjacent 
representative points is bounded by $\dfrac{L}{m}$. Let $R^O_{(I,s)}$ 
be a tour that is optimal. Let $R'_{(I,s)}(m)$ be a tour for the instance 
$(I,s)$ such that for an object $i$, $R^O_{(I,s)}$,visits the object 
at a representative point that is closest to the point on $i$ visited 
by $R^O_{(I,s)}$. It is easy to verify that any corresponding line
segments on  $R'_{(I,s)}(m)$ and $R^O_{(I,s)}$ cannot differ by 
more than $\dfrac{L}{m}$. Therefore, 
$$\|R_{(I,s)}(m)\| \leq \|R'_{(I,s)}(m)\|\leq OPT_{(I,s)} + \dfrac{|s|L}{m}.$$
\end{proof}
%\jy{I removed the min-cost flow thing which seems to be distracting.}

\begin{comment}
\subsection{Improvement with Minimum-Cost Flow}
To improve $R_{(I,s)}(m)$, a straightforward idea is adding more 
representative points. Denote $p_i$ as the pickup point of $R_{(I,s)}(m)$ 
on object i. For each object $i$ with perimeter $l_i$, we sample the 
($\dfrac{l_i}{2m})-$neighborhood of the pickup point $p_i$ with $m^*$ number of points. When $p_i$ is an endpoint of object $i$, the length of the new gap will be $\dfrac{l}{2(d-1)(d^*-1)}$; otherwise, the length will be $\dfrac{l}{(d-1)(d^*-1)}$. Moreover, we set the pickup sequence of the improved route the same as that of $R_{(I,s)}(d)$. Given the sequence, the new problem can be solved with a minimum-cost flow model.\\
\end{comment}
